Learning to Collocate Neural Modules for Image Captioning

We do not speak word by word from scratch; our brain quickly structures a pattern like \textsc{sth do sth at someplace} and then fill in the detailed descriptions. To render existing encoder-decoder image captioners such human-like reasoning, we propose a novel framework: learning to Collocate Neural Modules (CNM), to generate the `inner pattern' connecting visual encoder and language decoder. Unlike the widely-used neural module networks in visual Q\&A, where the language (ie, question) is fully observable, CNM for captioning is more challenging as the language is being generated and thus is partially observable. To this end, we make the following technical contributions for CNM training: 1) compact module design --- one for function words and three for visual content words (eg, noun, adjective, and verb), 2) soft module fusion and multi-step module execution, robustifying the visual reasoning in partial observation, 3) a linguistic loss for module controller being faithful to part-of-speech collocations (eg, adjective is before noun). Extensive experiments on the challenging MS-COCO image captioning benchmark validate the effectiveness of our CNM image captioner. In particular, CNM achieves a new state-of-the-art 127.9 CIDEr-D on Karpathy split and a single-model 126.0 c40 on the official server. CNM is also robust to few training samples, eg, by training only one sentence per image, CNM can halve the performance loss compared to a strong baseline.

==> ablative_studies.tex <==
For validating the significance of the proposed visual modular encoder, the module chosen block, and the stacking of the decoder units in the language decoder, we ablated our method with the following baselines:

\textbf{Base:} The encoder only contains the object module, and the decoder only contains one decoder unit without language module and module chosen block. This baseline provides a benchmark for other ablative baselines.

\textbf{Modules:} The encoder contains three visual modules, and the decoder only contains one decoder unit with language module, while module chosen block is not used. Compared with Base, the importance of the designed visual modules and language module can be validated.

\textbf{Modules+MC:} The designed three visual modules and language module are all implemented, and the decoder only includes one modular decoder unit with module chosen block. Compared with Modules, the importance of the module chosen block can be validated.

\textbf{Base+Deep:} Only object module is used, and the decoder includes multiple decoder units, while the module chosen block and language module are not used. The significance of stacking decoder units in language decoder can be demonstrated by comparing this baseline with Base.

\textbf{SAM w/o Expertise:} Compared with SAM, the expertise supervisions are not provided for training module chosen block. By comparing this baseline with SAM, the roles of explicitly using supervisions for guiding the module chosen can be discovered.

\noindent\textbf{Results and Analysis}.

\noindent\textbf{Qualitative Examples}.

\subsection{Comparisons with State-of-The-Arts}
\noindent\textbf{Comparing Methods}.
We only compared our SAM with recently proposed neural encoder-decoder based methods, because these methods own better performances than some more previous template or statistic based methods. The following models are chosen as comparisons: \textbf{Up-Down}~\cite{anderson2018bottom}, \textbf{LSTM-A}~\cite{yao2017boosting}, \textbf{SGAE}~\cite{yang2018auto}, \textbf{SCST}~\cite{rennie2017self}, \textbf{StackCap}~\cite{gu2017stack}, \textbf{CAVP}~\cite{liu2018context}, and \textbf{RFNet}~\cite{jiang2018recurrent}, whose encoders or decoders are improved by various techniques. Concretely, Up-Down, LSTM-A, and SGAE apply advanced encoders, \eg, Up-Down extracts enhanced visual features from ResNet based Faster R-CNN~\cite{ren2015faster}, while LSTM-A and SGAE explicitly incorporate high-level semantic knowledge in the encoder. SCST, StackCap, CAVP, and RFNet implement more complex training targets or decoder structures, \eg, SCST and StackCap design training targets upon Reinforcement Learning, while CAVP and RFNet use more LSTM layers in the decoder. Compared with these methods, our SAM not only enhances the encoder by using visual modules, but also equips the decoder unit with a complementary module chosen block, and further stacks these decoder units in a residual manner for multi-step reasoning for each word. 

\noindent\textbf{Human Evaluations}.
Automatic evaluations mainly concern the similarity between the generated captions with the human annotated captions. Though they are efficient and can measure the performances of captioning models, they neglect the descriptiveness, which can reflect the qualities of the generated captions~\cite{luo2018discriminability}. For achieving a more comprehensive evaluation of our SAM, we conducted human evaluation to compare the descriptiveness of the generated captions between SAM with SGAE. We chose SGAE as comparison since this model exploits language bias that the generated captions trend to own more details and thus the descriptiveness can be guaranteed. Also, such comparison is also conducted between SAM with Base.

Specifically, we showed two captions generated by different models and asked 30 workers that which one contains more details. For each pairwise comparison, we sampled 100 images from the Karpathy test set for workers to compare. The results of these comparisons are made as pie charts shown in Figure XXX.

\noindent\textbf{Results and Analysis}.




1. Module-O: similar to up-down
2. Module-A: similar to up-down with attribute feature
3. Module-R: similar to updown with relationship feature

The above shows each one has its own advantage, so, motivation is to stack them.

4. SAM with some single stacks internal tweaks? (why you design stack like that)

5. SAM with different length of stacks? (why residual blocks)

(all the above is normal RNN language decoder)

6. SAM-with different language decoder. RL, SGAE. (Transformer without transformer encoder cannot work well, or not consistent. Of course, SAM turns into transformer also ok but out of scope, future work)

7. Think of possible human eval for the above streams. 



State-of-the art, server, karparthy ......

==> experiments.tex <==
\section{Experiments}
\subsection{Dataset, Settings, and Metrics}
\noindent\textbf{MS-COCO~\cite{lin2014microsoft}.} 
COCO is the mainstream dataset for evaluating the performances of image captioning models that each image is assigned about 5 captions. This dataset provides one official split: 82,783, 40,504 and 40,775 images for training, validation and test respectively. For adjusting the hyper-parameters and offline test, the 3rd-party Karpathy split~\cite{karpathy2015deep} was also used, which has 113,287, 5,000, 5,000 images for training, validation and test respectively.

\noindent\textbf{Settings.} 


\noindent\textbf{Metrics.}
Five standard metrics were applied for evaluating the performances of the proposed method: CIDEr-D~\cite{vedantam2015cider}, BLEU~\cite{papineni2002bleu}, METEOR\cite{banerjee2005meteor}, ROUGE~\cite{lin2004rouge} and SPICE~\cite{anderson2016spice}.

\subsection{Ablative Studies}
\subsubsection{Architecture}
\noindent\textbf{Comparing Methods}.
For validating the significance of the proposed different modules, the module chosen/module interaction sub-block, and the deep structure of the modular decoder, we ablated our method with the following baselines:

\textbf{Obj:} The encoder only contains object module, and the decoder only contains two LSTMs without module chosen/module interaction sub-block.

%\textbf{Obj+Attr:} The encoder contains object and attribute modules, and the decoder only contains two LSTMs. This baseline is applied for validating the importance of the deployed attribute module.

\textbf{Obj+Attr+Rela:} The encoder contains all three modules, and the decoder only contains two LSTMs. Compared with baseline \textbf{Obj+Attr}, the importance of the relation module can be validated.

\textbf{Modules + MC/MI:} The encoder contains all three modules, and the decoder only includes one modular decoder block with module chosen/module interaction sub-block. Compared with baseline \textbf{Obj+Attr+Rela}, the importance of the module chosen/module interaction can be validated.

\textbf{MDB w/o MC/MI:} The encoder only contains object module, and the decoder includes multiple decoder blocks, while the module chosen/module interaction block is not used. Compared with baseline \textbf{Obj}, the importance of the MDB can be validated.

\begin{table}[t]
\begin{center}
\caption{The performances of various methods on MS-COCO Karpathy split. The metrics: B@N, M, R, C and S denote BLEU@N, METEOR, ROUGE-L, CIDEr-D and SPICE. The best results for each metric are marked in boldface separately.}
\label{table:tab_kap}
\scalebox{0.78}{
\begin{tabular}{l c c c c c c}
		\hline
		   Models   & B@1 & B@4 & M & R &  C & S\\ \hline
           SCST~\cite{rennie2017self}       & $-$  & $34.2$ & $26.7$ & $55.7$ & $114.0$ & $-$   \\ 
           LSTM-A~\cite{yao2017boosting}   & $78.6$  & $35.5$ & $27.3$ & $56.8$ & $118.3$ & $20.8$   \\ 
           StackCap~\cite{gu2017stack}    & $78.6$  & $36.1$ & $27.4$ & $-$ & $120.4$ & $-$   \\ 
           Up-Down~\cite{anderson2018bottom}  & $79.8$ & $36.3$ & $27.7$ & $56.9$ & $120.1$ & $21.4$ \\ 
           RFNet~\cite{jiang2018recurrent}  & $80.4$ & $37.9$ & $28.3$ & $58.3$ & $125.7$ & $21.7$ \\ 
           CAVP~\cite{liu2018context}  & $-$& $\mathbf{38.6}$ & $28.3$ & $58.5$ & $126.3$ & $21.6$ \\ \hline
           Base       & $79.9$ & $36.8$& $27.7$ & $57.0$ & $120.6$ & $20.9$\\ 
           Base+MGCN       & $80.2$ & $37.2$& $27.9$ & $57.5$ & $123.4$ & $21.2$\\ 
           Base+$\bm{D}$ w/o GCN       & $80.2$ & $37.3$& $27.8$ & $58.0$ & $124.2$ & $21.4$\\ 
           Base+$\bm{D}$       & $80.4$ & $37.7$& $28.1$ & $58.2$ & $125.7$ & $21.4$\\ 
           SGAE    & $\mathbf{80.8}$ & $38.4$ & $28.4$ & $\mathbf{58.6}$ & $\mathbf{127.8}$ & $\mathbf{22.1}$\\ \hline 
\end{tabular}
}
\end{center}
\end{table}

\begin{table*}[t]
\begin{center}
\caption{The performances of various methods on the online MS-COCO test server. The metrics: B@N, M, R, and C denote BLEU@N, METEOR, ROUGE-L, and CIDEr-D.}
\label{table:tab_online}
\scalebox{0.86}{
\begin{tabular}{l c c c c c c c c c c c c c c}
		\hline
		 Model & \multicolumn{2}{c}{B@1}  & \multicolumn{2}{c}{B@2}  & \multicolumn{2}{c}{B@3} & \multicolumn{2}{c}{B@4} &\multicolumn{2}{c}{M} &\multicolumn{2}{c}{R-L} & \multicolumn{2}{c}{C-D}\\ \hline 
		 Metric  &  c5 & c40 & c5 & c40 &  c5 & c40 & c5 & c40 & c5 & c40 & c5 & c40 & c5 & c40 \\ \hline
           SCST~\cite{rennie2017self}      & $78.1$ & $93.7$ & $61.9$ & $86.0$ & $47.0$ & $75.9$ & $35.2$ & $64.5$ & $27.0$ & $35.5$ & $56.3$ & $70.7$ & $114.7$ & $116.0$  \\
           LSTM-A~\cite{yao2017boosting}   & $78.7$ & $93.7$ & $62.7$ & $86.7$ & $47.6$ & $76.5$ & $35.6$ & $65.2$ & $27.0$ & $35.4$ & $56.4$ & $70.5$ & $116.0$ & $118.0$  \\ 
           StackCap~\cite{gu2017stack}     & $77.8$ & $93.2$ & $61.6$ & $86.1$ & $46.8$ & $76.0$ & $34.9$ & $64.6$ & $27.0$ & $35.6$ & $56.2$ & $70.6$ & $114.8$ & $118.3$   \\ 
           Up-Down~\cite{anderson2018bottom}    & $80.2$ & $95.2$ & $64.1$ & $88.8$ & $49.1$ & $79.4$ & $36.9$ & $68.5$ & $27.6$ & $36.7$ & $57.1$ & $72.4$ & $117.9$& $120.5$  \\ 
           CAVP~\cite{liu2018context}           & $80.1$ & $94.9$ & $64.7$ & $88.8$ & $50.0$ & $79.7$ & $37.9$ & $69.0$ & $28.1$ & $37.0$ & $58.2$ & $73.1$ & $121.6$& $123.8$    \\
           SGAE    & $80.6$ & $95.0$  & $65.0$ & $88.9$ & $50.1$  & $79.6$ & $37.8$ & $68.7$& $28.1$ & $37.0$ & $58.2$ & $73.1$ & $122.7$ & $125.5$\\ 
           \hline
\end{tabular}
}
\end{center}
\vspace{-0.1in}
\end{table*}

\subsubsection{Human Evaluation}


\subsubsection{Comparisons with State-of-The-Arts}

==> intro_temp.tex <==
%Why challenge (we need to collocate while generate the sentence, thus only partial information is given during collocation), Therefore, to enable effective training. We design simple modules and a controller loss. One or two sentence for each of them. Hightlight that Traditonal attention model is only a special case.



%We showcase:1) more accurate grammar: an/a: we disentangle the linguistic [is \&are], plural forms 2) more descriptive: adjective xxxxx.  3) more object interactions: quantity, verb like birds not neccesarrily flying in the sky.


%Overall, (experimental results show off)

%Contributions:

%1. first moduel networks for image captioning. This may complete the spectrum of using modules for vision language tasks. 

%2. we design a xxx loss for modules. 

%3. significant improvement has been made by using modules. potential research direction may follow how to design more reasonable modules for image captioning.


% how to reduce the diversity? Before we delve into the solution. Let's again try to describe the images, but this time, provided a sentence structure: STH DO STH. Perhaps most of you will not so far from the correct answer.  Cognitive science shows that we human learn to speak by patterns xxxxxxx. Point out the collocation. This is the neural modules.

% Neural modules are the solutions and they are not new in computer vision. When we struggle visual reasoning, we design modules, which are from questions. for example, we have xxxx. However, so far, we haven't observe a neural module network for image captioning. The challenge is that it is dynamically generated. 
% Due to this challenge, we design 1) simple generic neural modules: what are the four modules. 2) a controller loss which utilize the linguistic structure. 
% Before we going to delving into the details of CAM design in Section xxx. We would like to showcase some of the empirical benefits introduced by CAM. Three benefits. More details are in Section experiments.

% We conduct an extensive experiemts for xxxx. xxxxx

% In this paper, we attempt to try this and achieve empirically positive answer to reduce the diversity. That is, besides how to generate sentences, we learn how to collocate attention modules. [why we call it attention modules?since we use attentions.] As shown in Figure xxx, we have four modules, xxxx. How we design this four modules? To learn the modules, we design a (postag to module loss) that constrain the modules. This works as an inductive bias to the model. This model is: let each specialized to do their part professionally. (disentangle first, and then unify them, neural-symbolic models.). 

% Note that it is an end-to-end fashion, that is the collocation and the word generation is in the same architecture. and learn collocate and language model from sctrach. The key philosophy behind this design is that collcation is both visual and grammatical. That is, see relationships, sth. doing sths. and grammatical, xxx must follow a xxxx. 

% we demosntrate the experiments. 






% 1. relation more accurate, disentangle object context (brids must flying in sky) and xxxxx. 
% 1. more descriptive(accurate quantity, verb, adjective, an elephant). updown only focus on describe xxx. , explicitly encourage the model to follow the collocation. 

% CAM offers more reasoning not only improving the performance:

 

% Recall the game \textit{Filling in the Blanks} which junior kids usually play when they learn to speak. Figure XXX. When we want to speak a sentence, such as when we were writing this paper, a plausible approach is to first draft a template and then implement part by part. This is how our brain works (find cognitive evidence). Invariance.

% However, state-of-the-art image captioning does not work in a similar way. it predict one by one without structure. Therefore, the model cannot \textbf{disentangle} language bias and specific predictions. For example, (find some co-occurrence based errors), which is generally found in vision-language tasks. Not reasoning.
% %observe `a bird', then just say `a bird fly'. 
% %shortsighted, prefer to say ``one man and one man'' instead of ``two men''
% %cannot summary the image, cannot say ``busy street''
% %some grammar errors will appear: ``a apple'' instead of ``an apple''

% In this paper, we propose to xxxxx. (high-level idea, collocate modules)

% To the best of our knowledge, it is the first neural modules for image captioning. The reason why it is not as popular as in other tasks such as VQA is that it is not completed sentence. introducing our training technical contribution? such as output-aware controller, gubmel softmax? xxx



% However, modern image captioning models do not perform in that intuitive way. What does it do? Summarize.

% In this paper, inspired by the intuitive show and tell for our human being. Across many $<$image, sentence$>$ pairs, we expect a model that can learn to compose a structure for sentence and then specifically  We want to teach our model learning to how to s

==> model.tex <==
\section{Model}

\subsection{Motivation}
The target of image captioning is to automatically generate a suitable description sequence $\bm{w}_{1:T}$ about one given image $I$. Comparing with mainstream neural network based encoder-decoder captioning model, we introduce modular network for image captioning which motivated from the perspectives of representation learning and neuroscience. From a representation learning standpoint~\cite{bengio2013representation}, a good representation learner should be able to capture the posterior distribution of the underlying explanatory factors for the observed input. As one very specific application of representation learning, an image captioning model also demands this disentangling ability. From a neuroscience standpoint, humans exploit different regions of brain in processing vision signals and in reasoning (cite xxx). For generating an over-all description of an image, we human will not only list the objects we see, but also will assign suitable attributes for observed objects and conjecture objects' relationships by reasoning. This evidence also suggests us to develop different modules to process different types of information for composing a human style captions.

\subsection{An overview}
1.Encoder-Decoder mode: the general one and ours

The task of image captioning can be formulated as the learning of the joint distribution of one sequence $\bm{w}_{1:T}=\{w_1,w_2,...,w_T\}$ given one image $I$:
\begin{equation}
\label{eq:eq1}
    p(\bm{w}_{1:T}|I) = \prod_{t=1}^T{p(w_t|\bm{w}_{1:t-1},I)}. \\
\end{equation}
Here the chain rule is used to decompose the joint distribution into a series of distributions over each word. 

In a traditionally encoder-decoder based image captioning model, an encoder (usually a CNN) is performed to transform an image $I$ to a set of visual features $\bm{V}$, and an RNN based decoder is constructed for computing word distribution $p(w_t|\bm{w}_{1:t-1},\bm{V})$ at step $t$ given the previous word sequences $\bm{w}_{1:t-1}$ and visual features $\bm{V}$. In addition, attention technique is also implemented to dynamically combine visual features from $\bm{V}$ for generating next word.

Compared with some existing models, we simulate knowledge processing of humans that exploiting different modules to produce various representation sets for caption decoding. Specifically, object module, attribute module and relationship module are proposed for generating exclusive representation sets from image. Also, illuminated by~\cite{lu2017knowing}, we also implement a language module for generating words which can be reasoned from language context instead of image.


\subsection{Training Objective}
Given ground truth caption $\bm{w}_{1:T}^*$, the parameters of the whole model in Eq.~\eqref{eq:eq1} can be end-to-end learned by minimizing the cross-entropy loss:
\begin{equation}
    L_{XE} = -\sum_{t=1}^{T}{\log p(w^* | \bm{w}_{1:t-1}^*,I)},
\label{equ:equ_celoss}
\end{equation}
or by maximizing a reinforcement learning (RL) based reward~\cite{rennie2017self} as:
\begin{equation}
    R_{RL} = \mathbb{E}_{w_t^s \sim p(w_t)}[r(\bm{w}_{1:T}^s;\bm{w}_{1:T}^*)],
    \label{equ:equ_rlloss}
\end{equation}
where $r$ is a sentence-level metric for the sampled sentence $\bm{w}_{1:T}^s$ and the ground-truth $\bm{w}_{1:T}^*$, \eg, the CIDEr-D~\cite{vedantam2015cider} metric.

\subsection{Visual Modular Encoder}
\label{subsec:modules}

\subsubsection{Object Module}
The object module is one small network: a fully connected layer followed by a leaky ReLU activation. The inputs of this object module are the $d_{roi}$ dimensional RoI features extracted from the final layer of a ResNet-101 Faster R-CNN~\cite{ren2015faster}. Thus, these features can provide abundant knowledge about the objects' categories. The output feature set of this module is denoted as $\bm{V}_O$.

\subsubsection{Attribute Module}
The attribute module owns the same structure as the object module with different parameters. Another difference is that the inputs of the attribute module are RoI features from the third convolution block of the ResNet-101. In the experiment, we decreased the dimension of these features into $d_{roi}$ with an attribute classifier by using attribute annotations from VG dataset~\cite{krishna2017visual}. The applied attribute classifier is a network consists two fully connected layers with a ReLU activation in between. We did this because the knowledge for predicting attributes and categories are not consistent, and an additional fine tuning can augment certain attribute knowledge. The output feature set of this module is denoted as $\bm{V}_A$.

\subsubsection{Relation Module}
The relation module is built upon the multi-head self-attention layer~\cite{vaswani2017attention}, which can automatically seek the connections among two or more objects. And such connections or context clues would benefit the predictions of relationship words in image captions. 

Formally, assuming that the input of one multi-head self-attention layer is $\bm{R}=[\bm{r}_1,...,\bm{r}_N]^T$, which is an $N \times d_{roi}$ matrix of $N$ objects' RoI features as used in object module. Then each head vector is computed by a scaled dot-product:
\begin{equation}
    \text{head}_i(\bm{R})=\text{Softmax}( \frac{\bm{R}\bm{W}_i^1(\bm{R}\bm{W}_i^2)^T}{\sqrt{d_k}} )\bm{R}\bm{W}_i^3,
\end{equation}
where $\bm{W}_i^1, \bm{W}_i^2, \bm{W}_i^3$ are all $d_{roi} \times d_k$ trainable matrices, $d_k=d_{roi}/k$ is the dimension of each head vector, and $k$ is the number of heads. Then these $k$ heads are concatenated and projected to another space by linear transformation:
\begin{equation}
    \text{MH}(\bm{R}) = \text{Concat}(\text{head}_1,...,\text{head}_k)\bm{W}_{C},
\end{equation}
where $\bm{W}_{C} \in \mathcal{R}^{d_{roi}\times d_{roi}}$ is also a trainable matrix. Finally, these multi-head vectors are fed into a position-wise feed-forward network to get the output feature set $\bm{V}_R$. The position-wise feed-forward network used here consists of two fully connected layers with a ReLU activation layer in between.

(ONE FIGURE CONTAINS TWO SUB-FIGURES: ONE FOR REAL IMAGE, ONE FOR INTUITIVE EXPLANATION BY USING SIMPLE SHAPES)

\subsection{Modular Decoder}
\subsubsection{Overview of Modular Decoder}
The whole modular decoder include a few modular decoder blocks. Each modular decoder block contains two LSTMs and one module chosen component/module interaction sub-block. 

The input of the first LSTM at each time step is denoted as $\bm{u}_t^1$, which contains three components:
\begin{equation}
    \bm{u}_t^1=\text{Concat}(\bm{W}_e \sigma_t, \bar{\bm{v}}, \bm{h}_{t-1}^2),
\end{equation}
where the $\bm{W}_e \sigma_t$ is the learnable embedding of the previously generated word, $\bar{\bm{v}}$ is the concatenation of mean-pooled features of three modular feature sets: $\bar{\bm{v}}=\text{Concat}(\bar{\bm{v}}_O,\bar{\bm{v}}_A,\bar{\bm{v}}_R)$, and $\bm{h}_{t-1}^2$ is the previous output of the second LSTM. 

The output of the first LSTM $\bm{h}_t^1$ is fed into the module chosen sub-block/ module interaction sub-block for generating an re-mapped feature $\hat{\bm{v}}_t$ which contains the desired visual knowledge from outputs of three visual modules or non-visual knowledge from accumulated context. The details of the module chosen sub-block/module interaction sub-block are demonstrated in Section {xxx}. Then, such informative re-mapped feature $\hat{\bm{v}}_t$ is concatenated with the output of the first LSTM $\bm{h}_t^1$ to form the input of the second LSTM $\bm{u}_t^2$ as:
\begin{equation}
    \bm{u}_t^2=\text{Concat}(\bm{h}_t^1, \hat{\bm{v}}_t).
\end{equation}

Inspired by~\cite{arad2018compositional} that a deeper structure owns the ability of multi-step reasoning, and recently advances in the field of natural language processing where deep representations are frequently exploited~\cite{Peters:2018,devlin2018bert,vaswani2017attention}, we also implement a deep residual structure for multi-step reasoning and exploiting deep representation for generating better captions.

\subsubsection{Visual Modular Attention Component}
Attention technique is one mainstream improvement used to dynamically re-map visual features into more informative one for caption generation. Given three feature sets $\bm{V}_O$, $\bm{V}_S$, and $\bm{V}_R$ generated from three visual modules in Section~\ref{subsec:modules}, we apply an asynchronous/a synchronous attention technique for re-mapping them as three feature vectors: $\hat{\bm{v}}_O$, $\hat{\bm{v}}_S$, and $\hat{\bm{v}}_R$. 

Formally, given one $N \times d_v$ visual feature matrix $\bm{V}=[\bm{v}_1,...,\bm{v}_N]^T$ and one key vector $\bm{h}$, we can compute the soft attention weights $\bm{\alpha}$ as follows:
\begin{equation}
\label{equ:sum_att1}
    a_{i} = \bm{\omega}^T \text{tanh}(\bm{W}_v \bm{v}_i+\bm{W}_h \bm{h}),
\end{equation}
\begin{equation}
\label{equ:sum_att2}
    \bm{\alpha}=\text{softmax}(\bm{a}),
\end{equation}
where $\bm{\omega} \in \mathcal{R}^{1 \times d_a}$, $\bm{W}_v \in \mathcal{R}^{d_a \times d_v}$, and $\bm{W}_h \in \mathcal{R}^{d_a \times d_{h}}$ are all trainable parameters. Then we sum all the vectors in $\bm{V}$ by soft weights $\bm{\alpha}$ to get the re-mapped vector $\hat{\bm{v}}$:
\begin{equation}
\label{equ:sum_att3}
    \hat{\bm{v}}=\sum_{i=1}^N{\alpha_i \bm{v}_i}.
\end{equation}

(Asynchronous Attention:)
Here we apply Eq.~\eqref{equ:sum_att1}, Eq.~\eqref{equ:sum_att2}, and Eq.~\eqref{equ:sum_att3} to $\bm{V}_O$, $\bm{V}_S$, and $\bm{V}_R$ with different trainable matrices to get three re-mapped vectors $\hat{\bm{v}}_O$, $\hat{\bm{v}}_A$, and $\hat{\bm{v}}_R$, respectively. While the same key vector is used, which is the output of the first LSTM $\bm{h}_1$. 

This is one kind of asynchronous attention technique. (THE REASON OF USING ASYNCHRONOUS ATTENTION)

(Synchronous Attention:)
Here we set the visual feature set $\bm{V}$ as the concatenation of $\bm{V}_O$, $\bm{V}_S$, and $\bm{V}_R$: the element $\bm{v}$ of $\bm{V}$ is $\text{Concat}(\bm{v}_O, \bm{v}_A, \bm{v}_R)$. Thus, $d_v$ equals to $3d_{roi}$. And the output of the first LSTM $\bm{h}_1$ is chosen as the key vector. After computing soft weights, we apply Eq.~\eqref{equ:sum_att3} to get $\hat{\bm{v}}=\text{Concat}(\hat{\bm{v}}_O,\hat{\bm{v}}_A,\hat{\bm{v}}_R)$.

\subsubsection{Language Module}
As demonstrated in~\cite{lu2017knowing} that some words are non-visual, like ``the'' and ``of'', that they can be directly inferred from accumulated language contexts instead of visual clues. Thus, inspired by this, we also insert a language module into the modular decoder for providing purely language context. The implemented language module is one small network: a fully connected layer followed by a leaky ReLU activation. The input of this language module at time step $t$ is the cell state of the second LSTM in decoder at last time step $\bm{c}_2^{t-1}$, which accumulating abundant language knowledge.

\subsubsection{Controller}
\label{subsec:controller}
Motivated from the assumption that consecutive signals tend to be associated with each other and so their disentangled explanatory factors~\cite{bengio2013representation}, we build our controller upon LSTM~\cite{hochreiter1997long}.
This controller works to create the distribution over four modules. The input of this controller is the same as the first LSTM of the decoder, which is the accumulated context knowledge and the word of last time step. And the distribution $p(m)$ is computed as:

\noindent\textbf{Strategy 1:}
\begin{equation}
\label{eq:eq4}
    [\bm{h}_t,\bm{c}_t] = \text{LSTM}(w_t,I,[\bm{h}_{t-1},\bm{c}_{t-1}])
\end{equation}
\begin{equation}
\label{eq:eq5}
     p(m|\bm{w}_{1:t-1},I)=\text{Softmax}(\bm{W}_M \bm{h}_t)
\end{equation}


\subsubsection{Deep Residual Structure}

==> model_temp.tex <==
\subsection{A probabilistic model}
The task of image captioning can be formulated as the learning of the joint distribution of one sequence $\bm{w}_{1:T}=\{w_1,w_2,...,w_T\}$ given one image $I$:
\begin{equation}
\label{eq:eq1}
    p(\bm{w}_{1:T}|I) = \prod_{t=1}^T{p(w_t|\bm{w}_{1:t-1},I)}. \\
\end{equation}
For the distribution over one token $p(w_t|\bm{w}_{1:t-1},I)$, by introducing $M$ modules as hidden variables, we can further decompose this distribution as:
\begin{equation}
\label{eq:eq2}
    p(w_t|\bm{w}_{1:t-1},I) = \sum_{m=1}^M{p(w_t,m|\bm{w}_{1:t-1},I)}.
\end{equation}
By using Bayes Rule, we can rewrite $p(w_t|\bm{w_{1:t-1}},I)$ as:
\begin{equation}
\label{eq:eq3}
    p(w_t,m|\bm{w}_{1:t-1},I) = p(w_t|m,\bm{w}_{1:t-1},I) p(m|\bm{w}_{1:t-1},I).
\end{equation}
In this paper, we use a LSTM based controller to produce the distribution $p(m|\bm{w}_{1:t-1},I)$ over $M$ modules, which is discussed in~\ref{subsec:controller}. And neural network based encoder-decoders to model $M$ modules' word distribution $p(w_t|m,\bm{w}_{1:t-1},I)$. Specifically, these modules will own different structures or parameters, which is introduced in Section~\ref{subsec:modules}.


The task of image captioning is to generate a natural sentence $\mathcal{S}=\{s_1,s_2,...,s_T\}$ which should be consistent with the given image $\mathcal{I}$.

Most advanced image captioning models own an encoder-decoder structure with transformation technique, which can be formulated as:
\begin{equation} \label{equ:equ_ende}
\begin{aligned}
 \textbf{Encoder:} \quad  &\mathcal{V} \leftarrow \mathcal{I}, \\
 \textbf{Transform:} \quad  &\hat{\mathcal{V}} \leftarrow \mathcal{V}, \\
 \textbf{Decoder:} \quad & \mathcal{S} \leftarrow \hat{\mathcal{V}}. \\
\end{aligned}
\end{equation}

Figure~\ref{fig:3} (a) shows one typical encoder-decoder captioning model, which is called Up-Down~\cite{anderson2018bottom}. In this model, the encoder is a well pre-trained ResNet-101  Faster-RCNN~\cite{ren2015faster,he2016deep} for extracting features $\mathcal{V}$ of salient image regions. And the decoder contains two LSTM layers with an attention network. The first LSTM use context knowledge and image features to produce one index vector. And this index vector is input to attention network for transforming $\mathcal{V}$ to a more adapted vector $\hat{\bm{v}}$, which is then fed into the second LSTM followed by a softmax layer for generating a new word. With the assist of advanced visual features and attention mechanism, the generated captions are more consistent with the images by listing the appeared objects compared with some previous captioning models. 

However, captioning is not only about listing the objects but at least also need to describe other visual contents like attributes and relationships of objects. More importantly, human-like captioning also requires the model to compose these elements with suitable structures in harmony with human language's inductive bias.   

For achieving this goal, we propose the Collocate Attention Module (CAM) for image captioning. This model is shown in Figure~\ref{fig:3} (b), which also follows Encoder-Decoder pipeline, and can be summarized as:
\begin{equation} \label{equ:cam}
\begin{aligned}
 \textbf{Modular Encoder:} \quad  &\mathcal{V}_O,\mathcal{V}_A,\mathcal{V}_R \leftarrow \mathcal{I} \\
 \textbf{Collocation Transform:} \quad  &\hat{\mathcal{V}} \leftarrow \mathcal{V}_O,\mathcal{V}_A,\mathcal{V}_R \\
 \textbf{Multi-Step Decoder:} \quad & \mathcal{S} \leftarrow \hat{\mathcal{V}}_M \leftarrow ... \leftarrow \hat{\mathcal{V}}_1 \\
\end{aligned}
\end{equation}

Compared with Up-Down model, the modular encoder of our CAM (cf. Section~\ref{sec:modules}) includes object, attribute, and relation modules to extract features containing knowledge of objects' categories, attributes, and relations, respectively. By using these features, our model can disentangle the word generation from objects' categories, for example, disentangle the verb `flying' from object `bird'. 

And the decoder of our CAM (cf. Section~\ref{sec:decoder}) is the stacks of $M$ Collocate Attention Cells (CAC) with residual connections for multi-step reasoning. Each CAC has a similar structure as the decoder of Up-Down, which contains two LSTM layers and one transformation network. While we use a new transformation network called collocation network (cf. Section~\ref{subsec:col_net}) for generating the sentence with structure. Specifically, this collocation network will firstly decide which modules should be used and then generate the adapted vector. 
%By this manner, our model 

Given a dataset with human labeled captions $\mathcal{S}$ for images $\mathcal{I}$, we can train the whole model by minimizing the cross-entropy loss:
\begin{equation}
    L_{XE} = -\log P(\mathcal{S}^*),
\label{equ:equ_celoss}
\end{equation}
or by maximizing a reinforcement learning (RL) based reward~\cite{rennie2017self}:
\begin{equation}
    R_{RL} = \mathbb{E}_{\mathcal{S}^s \sim P(\mathcal{S})}[r(\mathcal{S}^s;\mathcal{S}^*)],
    \label{equ:equ_rlloss}
\end{equation}
where $r$ is a sentence-level metric for the sampled sentence $\mathcal{S}^s$ and the ground-truth $\mathcal{S}^*$, \eg, the CIDEr-D~\cite{vedantam2015cider} metric.




\subsection{Decoder with Modular Collocation}
\label{subsec:decoder}
In this section, we will introduce how collocation network chooses modules in Section~\ref{subsec:col_net}, and how multi-step reasoning is achieved by using multiple CACs in Section~\ref{subsec:ms_res}.
%In this section, we will introduce the decoder of our CAM model. As shown in Figure~\ref{fig:2} (b), the decoder includes $M$ CACs. Each CAC contains two LSTM layers and one collocation network in between, and residual connection is also applied. The input of each CAC at $t$ time step is the concatenation of three terms:
% \begin{equation}
%     \bm{x}_t = \text{Concat}(\bm{y}_t,\bar{\bm{v}},\bm{h}_{t-1}^2),
% \end{equation}
%where $\bm{y}_t$ is the output of previous CAC or learnable word embedding of generated word at last time step if this CAC is the first one among $M$ CACs, $\bar{\bm{v}}$ is the concatenation of mean-pooled features of three modular feature sets: $\bar{\bm{v}}=\text{Concat}(\bar{\bm{v}}_O,\bar{\bm{v}}_A,\bar{\bm{v}}_R)$, and $\bm{h}_{t-1}^2$ is the output of the second LSTM of this CAC at $t-1$ time step. 

%This input $x_t$ is also fed to the first LSTM, and also be connected to the output by residual shortcut. The output of the first LSTM $\bm{h}_{t-1}^1$ accumulates the context knowledge, and be used as the input of the collocation network for transforming visual features into one more adapted vector, as shown in Eq.~\eqref{equ:cam}.

%通过和bottom up对比来写，写自己的不同之处，一个不同是我们的decoder包含多个CAC，每个CAC和bottom up对比着写；还有一个是collocation network，可以让model有plan/structure的生成句子；
%把两个lstm的输出定义一下，可以在collocation network的时候用。

\subsection{Collocation Network}
\label{subsec:col_net}
Figure~\ref{fig:5} shows the detail of our collocation network. This network contains three attention network, one function module, and one controller. 

Three attention networks own the same structure as the one used in Bottom-Up~\cite{anderson2018bottom} with different parameters. $\mathcal{V}_O$, $\mathcal{V}_A$, and $\mathcal{V}_R$ are three feature sets extracted from three visual modules as discussed in Section~\ref{sec:modules}. And $\bm{h}_1^t$ is the output of the first LSTM layer of a CAC, as sketched in Figure~\ref{fig:3} (b). Three attended features can be got from these attention networks, which are $\hat{\bm{v}}_O^t$, $\hat{\bm{v}}_A^t$, and $\hat{\bm{v}}_R^t$ containing object, attribute, and relation knowledge about different regions of the image. As demonstrated in~\cite{lu2017knowing} that some words are functional that require few visual knowledge for inferring. Motivated by this, a function module is also proposed for directly generating these function words from accumulated context knowledge. The input of this module is $\bm{c}_t^2$, the cell state at last time step of the second LSTM of a CAC. It goes through a fully connected layer and the output is $\hat{\bm{v}_F^t}$.

Then, the controller will create four soft weights over four modules. Since the collocations of modules should be consecutive, for example, after generating an attribute word, it is more possible to generate an object word, we use a LSTM for generating soft weights at consecutive time steps. And at each time step, we provide accumulated context knowledge and visual clues of attended regions as the input for this LSTM, which is $\bm{x}_C^t$:
\begin{equation}
    \bm{x}_C^t=\text{Concat}(\bm{c}_2^{t-1},\hat{\bm{v}}_O^t,\hat{\bm{v}}_A^t,\hat{\bm{v}}_R^t).
\end{equation}
After generating soft weights $\bm{w}_t=\{w_O,w_A,w_R,w_F\}$ from the controller, we can have the adapted vector $\hat{\bm{v}}^t$ as:
\begin{equation}
    \hat{\bm{v}}^t=\text{Concat}(w_O\hat{\bm{v}}_O^t,w_A\hat{\bm{v}}_A^t,w_R\hat{\bm{v}}_R^t,w_F\hat{\bm{v}}_F^t).
\end{equation}
%1.each module attended to specific region, and the attended feature of each feature contains different knowledge for generating different words
%2.instead of directly generating one word, collocation network first decide which kind of word should be generated
%3.thus, our model do not generate one word immediately after finding a region, while choosing the most suitable one among four options.
%在生成一个词的时候，可以有不同的选择，3个不同的visual modules可以看到不同的image region，func module意味着可以直接从context生成一个func word。所以我们的model可以有计划的生成句子，先选module，后生成word。这是一种with structure的方式。

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 5mm 5mm 5mm,clip]{latex/fig_col.pdf}
   \caption{}
\label{fig:5}
\end{figure}
\subsection{Multi-step Reasoning}
\label{subsec:ms_res}
%model需要观察到足够的信息才能做出最终的module的选择，所以我们提出了multi-step reasoning。同时，我们李永乐residual 结构，这样一来，如果前面选择的module已经足够好了，那么这些信息可以直接通过shotcut传递到最后的决策层去生成word。



%Motivated by the observations from cognitive science~\cite{xxx} that humans' brain use different regions for transforming visual information into various high level semantic knowledge. We also design three visual modules and encourage each one to learn exclusive knowledge, \ie, the object module captures object categories about image regions for generating nouns, the attribute module captures attribute labels for generating adjectives, and the relation module captures interactions among objects for generating verbs, prepositions or quantifiers. By encouraging each visual module to focus more on their exclusive knowledge, our CNM can disentangle caption generation from dataset bias like high co-occurrence frequency of certain word combinations. For example, our CNM will generate the accurate relation ``bird-perch-tree'' only when the relation module recognizes the action ``perch'', instead of generating verb ``fly'' like Up-Down caused by high co-occurrence frequency between ``bird'' and ``fly'' in training set, such an example is shown in Figure~\ref{fig:rela} (b).

%We apply the following techniques for encouraging each visual module to learn exclusive knowledge: 1) different pre-training strategies are deployed for three visual modules, 2) the relation module is built upon multi-head self-attention mechanism for automatically seeking interactions among objects, 3) an additional linguistic controller loss is designed for instructing each module to learn exclusive knowledge about the related word. The former two techniques will be introduced in this section, and the linguistic controller loss will be discussed in Section~\ref{subsec:controller}.
%两种structure的module，一种是singular，一种是pairwise

% Formally, assuming that the input of one multi-head self-attention layer is $\bm{R}=[\bm{r}_1,...,\bm{r}_N]^T$, which is a $N \times d_{roi}$ matrix of $N$ objects' RoI features as used in object module. Then each head vector is computed by a scaled dot-product:
% \begin{equation}
%     \text{head}_i(\bm{R})=\text{Softmax}( \frac{\bm{R}\bm{W}_i^1(\bm{R}\bm{W}_i^2)^T}{\sqrt{d_k}} )\bm{R}\bm{W}_i^3,
% \end{equation}
% where $\bm{W}_i^1, \bm{W}_i^2, \bm{W}_i^3$ are all $d_{roi} \times d_k$ trainable matrices, $d_k=d_{roi}/k$ is the dimension of each head vector, and $k$ is the number of heads. Then these $k$ heads are concatenated and projected to another space by linear transformation:
% \begin{equation}
%     \text{MH}(\bm{R}) = \text{Concat}(\text{head}_1,...,\text{head}_k)\bm{W}_{C},
% \end{equation}
% where $\bm{W}_{C} \in \mathcal{R}^{d_{roi}\times d_{roi}}$ is also a trainable matrix. Finally, these multi-head vectors are fed into a position-wise feed-forward network to get the output feature set $\mathcal{V}_R$. The position-wise feed-forward network consists of two fully connected layers with a ReLU activation layer in between.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 5mm 5mm 5mm,clip]{latex/fig_rela.pdf}
   \caption{}
\label{fig:rela}
\end{figure}

==> related_work.tex <==
\section{Related Work}
\subsection{Image Caption}
Automatically generating a natural description about an image has for decades attracted researchers' attentions. Before the pervasive application of deep networks, most of caption models belong to rule/template or statistic based methodology~\cite{kuznetsova2012collective,mitchell2012midge,li2011composing,kulkarni2011baby}.
Nowadays, a majority of deep learning based image captioning methods are deployed by simulating the process of human captioning. In~\cite{vinyals2015show}, the image is mapped into one kind of middle representations and then these representations are decoded for caption generation, just like we humans firstly encode visual information by visual system and then exploit brain to produce the corresponding description.
Also, by observing the facts that when we humans describe one image, we usually describe the regions one by one of that image in some sort of order, various attention techniques ~\cite{xu2015show,lu2017knowing,anderson2018bottom,liu2018context} are proposed. By using them, different regions of image will be dynamically concentrated on when each new word is generated.

For further improving the quality of the generated captions, some research begin to directly incorporate high-level semantic information into encoder-decoder pipeline, \eg, object categories~\cite{lu2018neural}, objects' attributes~\cite{yao2017boosting}, objects' pairwise relationships~\cite{yao2018exploring} or scene graphs~\cite{yang2018auto}.

\subsection{Modular Network}



